SN 1987A : Tracing the flux decline and spectral evolution through a comparison of SRG/eROSITA and XMM-Newton observations

SN 1987A is the closest observed supernova in the last four centuries and provides a unique opportunity to witness the birth and evolution of a supernova remnant. The source has been monitored by XMM Newton EPIC-pn from 2007--2020. SRG/eROSITA also observed the source during its commissioning phase and the first light in Sept. and Oct. 2019. We investigated the spectral and flux evolution of SN 1987A in X-rays over the last fourteen years up to Nov. 2020 using XMM-Newton and eROSITA observations. We performed a detailed spectral analysis using a three-component plane-parallel shock model and analysed and modelled the EPIC-pn monitoring and eROSITA observations in a consistent manner. This paper reports a complete and most up to date flux evolution of SN 1987A in the soft (0.5-2 keV) and hard (3-10 keV) X-ray band. The flux in the soft band flattened around 9424 d and then displayed a turnover between 10142-10493 d after which it showed a continued decline. Around the same time, a break in the hard-band flux time evolution slope was detected. This implies that the blast wave has now passed beyond the dense structures of the equatorial ring and is expanding further into more tenuous circumstellar medium. The temporal evolution of the normalizations of the three shock components match well the results of hydrodynamical simulations predicting a blue supergiant progenitor scenario. The trend at recent epochs indicate that the emission caused by the forward shock after leaving the equatorial ring and by the reverse shock in the ejecta is becoming more dominant now. The elemental abundances in the hot plasma component are significantly higher than those in the `cooler' one, indicating its origin from the reverse shock propagating into the ejecta.

==> SN1987A_EPICpn_flux.tex <==

% ---------------------------------------------------------------------------
% Table : Details of XMM obs. 
% ---------------------------------------------------------------------------
\begin{table*}
\caption{Details of the XMM-Newton EPIC-pn observations}
\label{table_EPICobs}
\centering
\begin{tabular}{lcccrr}
\hline\hline
\noalign{\smallskip}
ObsId & Obs. start date & Age \tablefootmark{a} & Exp. times \tablefootmark{b} & Flux (0.5--2 keV) & Flux (3--10 keV) \\
      &                 & (days) & (ks) & \multicolumn{2}{c}{$\left(10^{-13}\right.$ erg\,s$^{-1}$\,cm$\left.^{-2}\right)$} \\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
% updated 2021-02-16 with latest fit results
0406840301 & 2007-01-17 &  7269 & 106.9/93.1 & 33.80$^{+0.87}_{-0.77}$ &  4.18$^{+0.27}_{-0.52}$ \\ \noalign{\smallskip}
0506220101 & 2008-01-11 &  7629 & 109.4/89.4 & 43.96$^{+1.01}_{-0.91}$ &  5.48$^{+0.31}_{-0.39}$ \\ \noalign{\smallskip}
0556350101 & 2009-01-30 &  8013 & 100.0/86.7 & 53.28$^{+1.06}_{-0.93}$ &  6.49$^{+0.35}_{-0.43}$ \\ \noalign{\smallskip}
0601200101 & 2009-12-12 &  8329 &  89.9/77.5 & 59.70$^{+0.69}_{-0.74}$ &  7.25$^{+0.40}_{-0.61}$ \\ \noalign{\smallskip}
0650420101 & 2010-12-12 &  8693 &  64.0/55.9 & 66.55$^{+0.89}_{-0.73}$ &  8.45$^{+0.47}_{-0.62}$ \\ \noalign{\smallskip}
0671080101 & 2011-12-02 &  9049 &  80.6/70.2 & 71.25$^{+0.70}_{-0.55}$ & 10.16$^{+0.49}_{-0.59}$ \\ \noalign{\smallskip}
0690510101 & 2012-12-11 &  9424 &  68.0/60.5 & 74.93$^{+0.64}_{-0.52}$ & 11.59$^{+0.57}_{-0.77}$ \\ \noalign{\smallskip}
0743790101 & 2014-11-29 & 10142 &  77.6/67.8 & 74.85$^{+0.50}_{-0.63}$ & 13.35$^{+0.55}_{-0.59}$ \\ \noalign{\smallskip}
0763620101 & 2015-11-15 & 10493 &  64.0/56.9 & 73.87$^{+0.66}_{-0.56}$ & 14.76$^{+0.66}_{-0.81}$ \\ \noalign{\smallskip}
0783250201 & 2016-11-02 & 10846 &  72.4/63.3 & 71.61$^{+0.57}_{-0.55}$ & 15.22$^{+0.61}_{-0.70}$ \\ \noalign{\smallskip}
0804980201 & 2017-10-15 & 11193 &  68.7/59.1 & 69.76$^{+0.49}_{-0.61}$ & 15.66$^{+0.55}_{-0.58}$ \\ \noalign{\smallskip}
0852980101 & 2019-09-06 & 11884 &  14.7/12.4 & 64.58$^{+1.32}_{-0.97}$ & 16.75$^{+1.27}_{-1.46}$ \\ \noalign{\smallskip}
0862920201 & 2020-11-24 & 12329 &  74.2/60.5 & 61.78$^{+0.67}_{-0.57}$ & 16.97$^{+0.50}_{-0.53}$ \\ \noalign{\smallskip}
\hline
\label{tabobsxmm}
\end{tabular}
\tablefoot{All observations were operated with the EPIC-pn camera in full-frame read-out
mode with the medium optical blocking filter. 
Fluxes are given with 90\% confidence range and are not corrected for absorption.
\tablefoottext{a}{Number of days since the explosion of SN\,1987A.}
\tablefoottext{b}{Total/filtered exposure times (after removal of high background intervals).}
}
\end{table*}

